Stout: Cloudy's Atomic and Molecular Database

We describe a new atomic and molecular database we developed for use in the spectral synthesis code Cloudy. The design of Stout is driven by the data needs of Cloudy, which simulates molecular, atomic, and ionized gas with kinetic temperatures 2.8 K < T < 1e10 K and densities spanning the low to high-density limits. The radiation field between photon energies $10^{-8}$ Ry and 100 MeV is considered, along with all atoms and ions of the lightest 30 elements, and ~100 molecules. For ease of maintenance, the data are stored in a format as close as possible to the original data sources. Few data sources include the full range of data we need. We describe how we fill in the gaps in the data or extrapolate rates beyond their tabulated range. We tabulate data sources both for the atomic spectroscopic parameters and for collision data for the next release of Cloudy. This is not intended as a review of the current status of atomic data, but rather a description of the features of the database which we will build upon.

==> LocalMacros.tex <==
% put new macros in this file for eventual export to master file

